Search for the Wh Production Using High-pT Isolated Like-Sign Dilepton Events in Run-II with 1.9 /fb

We search for the neutral higgs production associated with the $W$ boson using high-$p_{T}$ isolated like-sign dilepton events in $p\bar{p}$ collisions at $\sqrt{s}$ = 1.96 TeV. The data were collected with the CDF-II detector at the Fermilab Tevatron collider and correspond to an integrated luminosity of 1.9 ${\rm fb}^{-1}$. We examine the dilepton events on the plane of the 2nd lepton $p_{T}$ ($p_{T2}$) versus the $ p_{T}$ of dilepton system ($p_{T12}$) and tune the final cut to maximize the sensitivity on the plane. We set the final cut to the 2nd lepton $p_{T}$ greater than 20 GeV/c and the $p_{T}$ of dilepton system greater than 15 GeV/c. The expected number of signal events is 0.46 for the fermiophobic higgs of the mass 110 GeV/$c^{2}$ and 0.19 for the mass 160 GeV/$c^{2}$ assuming the Standard Model cross section. The number of events for the Standard Model higgs is 0.02 and 0.18 for 110 GeV/$c^2$ and 160 GeV/$c^{2}$, respectively. The expected number of backgrounds is 3.23 $\pm$ 0.69, while we observed 3 events in the data. From these results, we obtain the limits on $\sigma(p\bar{p}\to Wh) \times Br(h\to W^{+}W^{-})$ of 2.2 pb for the higgs of 110 GeV/$c^{2}$ and 1.4 pb for 160 GeV/$c^2$ at the 95% confidence level.

==> Makefile <==
###############################################################################
#                                                        December 4, 2002
#
# Makefile for a sample CDF Note - Stefan Stonjek  <s.stonjek@physics.ox.ac.uk>
#                                  Martin Hennecke <hennecke@fnal.gov> 
#
###############################################################################

graphics_eps := $(wildcard *.eps)
graphics_pdf := $(patsubst %.eps,%.pdf,$(wildcard *.eps))

target=slacconf_one
ps: $(target).ps
	gv $(target).ps

pdf: $(target).pdf
	acroread $(target).pdf

$(target).pdf: $(target).tex $(graphics_pdf)
	pdflatex $(target).tex && pdflatex $(target).tex && thumbpdf $(target) && pdflatex $(target).tex

$(target).ps: $(target).tex
	latex $(target).tex && latex $(target).tex && dvips $(target).dvi -o 

%.pdf: %.eps
	ps2pdf $< $@

.PHONY: clean
clean:
	rm -r -f $(target).aux $(target).dvi $(target).log $(target).out $(target).pdf \
	$(target).ps $(target).toc $(target).tof thumb*.* *~ $(graphics_pdf)

